All crepant resolutions of hyperpolygon spaces via their Cox rings

We construct and enumerate all crepant resolutions of hyperpolygon spaces, a family of conical symplectic singularities arising as Nakajima quiver varieties associated to a star-shaped quiver. We provide an explicit presentation of the Cox ring of any such crepant resolution. Using techniques developed by Arzhantsev-Derenthal-Hausen-Laface we construct all crepant resolutions of the hyperpolygon spaces, including those which are not projective over the singularity. We find that the number of crepant resolutions equals the Ho\c{s}ten-Morris numbers. In proving these results, we obtain a description of all complete geometric quotients associated to the classical GIT problem constructing moduli spaces of ordered points on the projective line. These moduli spaces appear as the Lagrangian subvarieties of crepant resolutions of hyperpolygon spaces fixed under the conical action.

==> notation.tex <==
\newpage
\section{Notation}

$n$: Fixed integer $\geq 5$.

$Q$: Star-shaped quiver with $n$ vertices.

$G$: Change of basis group $\GL(Q)/\CC^*$. (General reductive group).

$T$: Torus $G/\SL(2)$.

$\Theta$: element of $G^\vee\otimes_\ZZ \QQ$, identified with $T^\vee\otimes_\ZZ\QQ$.

$F$: positive orthant of $\Theta$ under the fixed choice of basis, fundamental domain for the Namikawa-Weyl group.

$\mathcal{X}$: Spectrum of the `pre' Cox ring.

$X$: $\Spec(\Cox(\MM))$.

$\mathcal{Y}$: $\Rep(Q,v)$.

$Y$: $\mathcal{Y}\git\SL_2$.

$V$: DUAL of the standard 2-dimensional representation of $\GL(2)$ or $\SL(2)$.

$P$: A partition of $[n]$.
